Dating ancient manuscripts using radiocarbon and AI-based writing style analysis

Determining the chronology of ancient handwritten manuscripts is essential for reconstructing the evolution of ideas. For the Dead Sea Scrolls, this is particularly important. However, there is an almost complete lack of date-bearing manuscripts evenly distributed across the timeline and written in similar scripts available for palaeographic comparison. Here, we present Enoch, a state-of-the-art AI-based date-prediction model, trained on the basis of new radiocarbon-dated samples of the scrolls. Enoch uses established handwriting-style descriptors and applies Bayesian ridge regression. The challenge of this study is that the number of radiocarbon-dated manuscripts is small, while current machine learning requires an abundance of training data. We show that by using combined angular and allographic writing style feature vectors and applying Bayesian ridge regression, Enoch could predict the radiocarbon-based dates from style, supported by leave-one-out validation, with varied MAEs of 27.9 to 30.7 years relative to the radiocarbon dating. Enoch was then used to estimate the dates of 135 unseen manuscripts, revealing that 79 per cent of the samples were considered 'realistic' upon palaeographic post-hoc evaluation. We present a new chronology of the scrolls. The radiocarbon ranges and Enoch's style-based predictions are often older than the traditionally assumed palaeographic estimates. In the range of 300-50 BCE, Enoch's date prediction provides an improved granularity. The study is in line with current developments in multimodal machine-learning techniques, and the methods can be used for date prediction in other partially-dated manuscript collections. This research shows how Enoch's quantitative, probability-based approach can be a tool for palaeographers and historians, re-dating ancient Jewish key texts and contributing to current debates on Jewish and Christian origins.

==> tables/TableX-1yrRes.tex <==
\footnotesize
\LTcapwidth=\textwidth
{\tabcolsep=3.3pt
\begin{longtable}{l|l|l|l|l|l}

\caption{Summarized results of 26 accepted \textsuperscript{14}C dates: laboratory code, sample identification, \textsuperscript{14}C age (BP), sigma (BP), calibrated ranges (1$\sigma$ and 2$\sigma$ ranges)}
\label{tab:summarized-c14}\\


\hline\hline 
\multirow{2}{*}{\textbf{lab code}} &
  \multirow{2}{*}{\textbf{scroll}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{age}\\ \textbf{(BP)}\end{tabular}} &
  \multirow{2}{*}{\textbf{$\sigma$}} &
  \multirow{2}{*}{\textbf{calibrated ranges (1$\sigma$)}} &
  \multirow{2}{*}{\textbf{calibrated ranges (2$\sigma$)}} \\
 &
   &
   &
   &
   &
   \\ \hline
GrA-68446 &
  P421-Fr004 &
  \multirow{3}{*}{2164} &
  \multirow{3}{*}{16} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}342–321, \\ 201–175 BCE\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}352–287, 228–219 BCE \end{tabular}} \\ %\\ 211–151 BCE%
GrA-68447 &
  \begin{tabular}[c]{@{}l@{}}4Q504 \\ (4QDibHam\textsuperscript{a})\end{tabular} &
   &
   &
   &
   \\ \hline
GrA-69793 &
  P206-Fr003 &
  \multirow{3}{*}{2303} &
  \multirow{3}{*}{26} &
  \multirow{3}{*}{401–369 BCE} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}407–356, \\ 281–232 BCE\end{tabular}} \\
GrM-10677 &
  4Q52 (4QSam\textsuperscript{b}) &
   &
   &
   &
   \\
GrM-10678 &
   &
   &
   &
   &
   \\ \hline
GrA-69794 &
  P285-Fr002 &
  \multirow{3}{*}{2153} &
  \multirow{3}{*}{19} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}343–321, \\ 202–166 BCE\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}351–304, 209–102, \\ 67–60 BCE\end{tabular}} \\
GrM-10679 &
  4Q176 (4QTanh) &
   &
   &
   &
   \\
GrM-10680 &
   &
   &
   &
   &
   \\ \hline
GrA-69795 &
  P224-Fr001 &
  \multirow{5}{*}{2168} &
  \multirow{5}{*}{15} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}343–320, \\ 202–176 BCE\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}352–287, 228–219, \\ 211–160 BCE\end{tabular}} \\
GrM-13252 &
  4Q114 (4QDan\textsuperscript{c}) &
   &
   &
   &
   \\
GrM-13253 &
   &
   &
   &
   &
   \\
GrM-13254 &
   &
   &
   &
   &
   \\
GrM-13255 &
   &
   &
   &
   &
   \\ \hline
GrM-10659 &
  P891-Fr003 &
  \multirow{2}{*}{1940} &
  \multirow{2}{*}{28} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}30–42,\\  59–124 CE\end{tabular}} &
  \multirow{2}{*}{10–204 CE} \\
GrM-10660 &
  5/6Hev1b (Ps) &
   &
   &
   &
   \\ \hline
GrA-69810 &
  P585-Fr001 &
  \multirow{3}{*}{2028} &
  \multirow{3}{*}{18} &
  \multirow{3}{*}{45 BCE–8 CE} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}89–80 BCE, \\ 54 BCE–27 CE, \\ 48–57 CE\end{tabular}} \\
GrM-10661 &
  4Q161 (4QpIsa\textsuperscript{a}) &
   &
   &
   &
   \\
GrM-10662 &
   &
   &
   &
   &
   \\ \hline
GrM-11151 &
  P1111-Fr010 &
  \multirow{4}{*}{2226} &
  \multirow{4}{*}{17} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}362–351, \\ 295–272, \\ 266–209 BCE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}375–346, \\ 317–203 BCE\end{tabular}} \\
GrM-11152 &
  4Q70 (4QJer\textsuperscript{a})\footnotemark{} &
   &
   &
   &
   \\
GrM-11170 &
   &
   &
   &
   &
   \\
GrM-11171 &
   &
   &
   &
   &
   \\ \hline
GrM-11153 &
  P1093-Fr005 &
  \multirow{3}{*}{2155} &
  \multirow{3}{*}{19} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}343–320, \\ 202–167 BCE\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}351–291, \\ 209–104 BCE\end{tabular}} \\
GrM-11154 &
  4Q47 (4QJosh\textsuperscript{a}) &
   &
   &
   &
   \\
GrM-11172 &
   &
   &
   &
   &
   \\ \hline
GrM-11155 &
  P271-Fr002 &
  \multirow{3}{*}{2152} &
  \multirow{3}{*}{24} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}346–316, \\204–151, \\ 129–123 BCE\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}351–289, 227–220, \\ 210–97, 71–58 BCE\end{tabular}} \\
GrM-11156 &
  4Q23 (4QLevNum\textsuperscript{a}) &
   &
   &
   & \\
   &
   &
   &
   &
   &
   \\ \hline
GrM-11166 &
  P177-Fr001 &
  \multirow{6}{*}{2100} &
  \multirow{6}{*}{17} &
  \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}152–94, \\74–56 BCE\end{tabular}} &
  \multirow{6}{*}{167–51 BCE} \\
GrM-11167 &
  \begin{tabular}[c]{@{}l@{}}4Q255/4Q433a \\ (4QpapS\textsuperscript{a}/4Qpap\\ Hodayot-like Text B)\end{tabular} &
   &
   &
   &
   \\
GrM-11184 &
   &
   &
   &
   &
   \\
GrM-11185 &
   &
   &
   &
   &
   \\ \hline
GrM-11168 &
  P977-Fr004 &
  \multirow{4}{*}{1967} &
  \multirow{4}{*}{18} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}23–78, \\ 101–107 CE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}31–16 BCE, \\ 7–120 CE\end{tabular}} \\
GrM-11169 &
  11Q5 (11QPs\textsuperscript{a}) &
   &
   &
   &
   \\
GrM-11186 &
   &
   &
   &
   &
   \\
GrM-11187 &
   &
   &
   &
   &
   \\ \hline
GrM-14380 &
  P393-Fr005 &
  \multirow{4}{*}{2123} &
  \multirow{4}{*}{21} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}174–102, \\ 67–60 BCE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}339–326, 199–89, \\ 81–53 BCE\end{tabular}} \\
GrM-14381 &
  4Q3 (4QGen\textsuperscript{c}) &
   &
   &
   &
   \\
GrM-14228 &
   &
   &
   &
   &
   \\
GrM-14229 &
   &
   &
   &
   &
   \\ \hline
GrM-13385 &
  P1081a-Fr002 &
  \multirow{2}{*}{2115} &
  \multirow{2}{*}{26} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}171–97, \\ 72–57 BCE\end{tabular} } &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}336–330, \\ 198–50 BCE\end{tabular}} \\
GrM-13386 &
  4Q27 (4QNum\textsuperscript{b}) &
   &
   &
   &
   \\ \hline
GrM-13387 &
  Px232-Fr001 &
  \multirow{4}{*}{2007} &
  \multirow{4}{*}{18} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}41–9 BCE,\\ 1 BCE–25 CE\end{tabular}} &
  \multirow{4}{*}{46 BCE–62 CE} \\
GrM-13388 &
  Mas1k (MasShirShabb) &
   &
   &
   &
   \\
GrM-14175 &
   &
   &
   &
   &
   \\
GrM-14223 &
   &
   &
   &
   &
   \\ \hline
GrM-14382 &
  P386-Fr001 &
  \multirow{4}{*}{2169} &
  \multirow{4}{*}{21} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}348–312, \\ 206–171 BCE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}356–281, 232–150, \\ 131–121 BCE\end{tabular}} \\
GrM-14383 &
  4Q206 (4QEn\textsuperscript{e} ar) &
   &
   &
   &
   \\
GrM-14230 &
   &
   &
   &
   &
   \\
GrM-14241 &
   &
   &
   &
   &
   \\\hline
GrM-14565 &
  P237-Fr007 &
  \multirow{5}{*}{2182} &
  \multirow{5}{*}{18} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}351–295 \\ 209–176 BCE\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}356–279, 256–248,  \\ 233–169 BCE\end{tabular}} \\
GrM-14566 &
  \begin{tabular}[c]{@{}l@{}}4Q30 (4QDeut\textsuperscript{c})\end{tabular} &
   &
   &
   &
   \\
GrM-14395 &
   &
   &
   &
   &
   \\
GrM-14242 &
   &
   &
   &
   &
   \\
GrM-14243 &
   &
   &
   &
   &
   \\ \hline
GrM-13389 &
  P904-Fr009 &
  \multirow{4}{*}{2077} &
  \multirow{4}{*}{18} &
  \multirow{4}{*}{107–46 BCE} &
  \multirow{4}{*}{162–41, 9–2 BCE} \\
GrM-13390 &
  \begin{tabular}[c]{@{}l@{}}4Q201/4Q338 \\ (4QEn\textsuperscript{a} ar/\\ 4QGenealogical List)\end{tabular} &
   &
   &
   &
   \\
GrM-14173 &
   &
   &
   &
   &
   \\
GrM-14174 &
   &
   &
   &
   &
   \\ \hline
GrM-14396 &
  P810-Fr011 &
  \multirow{4}{*}{2148} &
  \multirow{4}{*}{19} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}343–322, \\ 201–155 BCE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}349–311, 206–100,\\  68–59 BCE\end{tabular}} \\
GrM-14397 &
  4Q259 (4QS\textsuperscript{e}) &
   &
   &
   &
   \\
GrM-14244 &
   &
   &
   &
   &
   \\
GrM-14245 &
   &
   &
   &
   &
   \\ \hline
GrM-14398 &
  P180-Fr004 &
  \multirow{5}{*}{2130} &
  \multirow{5}{*}{22} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}196–184, \\ 179–104 BCE\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}343–321, 202–91,\\  79–54 BCE\end{tabular}} \\
GrM-14399 &
    \begin{tabular}[c]{@{}l@{}}4Q416 \\(4QInstruction\textsuperscript{b})\end{tabular} &
   &
   &
   &
   \\
GrM-14246 &
   &
   &
   &
   &
   \\
GrM-14359 &
   &
   &
   &
   &
   \\ \hline
GrM-14400 &
  P215-Fr004 &
  \multirow{4}{*}{2059} &
  \multirow{4}{*}{20} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}97–71, \\ 58–39, \\ 11 BCE–2 CE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}152–131 BCE, \\ 121 BCE–10 CE\end{tabular}} \\
GrM-14401 &
  4Q2 (4QGen\textsuperscript{b}) &
   &
   &
   &
   \\
GrM-14360 &
   &
   &
   &
   &
   \\
GrM-14361 &
   &
   &
   &
   &
   \\ \hline
GrM-14567 &
  P122A-Fr001 &
  \multirow{4}{*}{2126} &
  \multirow{4}{*}{23} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}193–189, \\176–101, \\ 67–60 BCE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}342–323, 201–88, \\ 82–53 BCE\end{tabular}} \\
GrM-14568 &
  \begin{tabular}[c]{@{}l@{}}4Q375 \\(4QapocrMoses\textsuperscript{a})\end{tabular} &
   &
   &
   &
   \\
GrM-14362 &
   &
   &
   &
   &
   \\
GrM-14363 &
   &
   &
   &
   &
   \\ \hline
GrM-13391 &
  P534-Fr002 &
  \multirow{5}{*}{1998} &
  \multirow{5}{*}{20} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}38–13 BCE, \\3–29, \\ 43–59 CE\end{tabular}} &
  \multirow{5}{*}{45 BCE–75 CE} \\
GrM-13392 &
  \begin{tabular}[c]{@{}l@{}}XHev/Se2 \\ (XHev/Se Num\textsuperscript{a})\end{tabular} &
   &
   &
   &
   \\
GrM-14224 &
   &
   &
   &
   &
   \\
GrM-14225 &
   &
   &
   &
   &
   \\ \hline
GrM-14569 &
  P147-Fr019 &
  \multirow{5}{*}{2148} &
  \multirow{5}{*}{22} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}343–320, \\ 202–152 BCE\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}351–305, 209–95, \\ 73–57 BCE\end{tabular}} \\
GrM-14570 &
    \begin{tabular}[c]{@{}l@{}}4Q541 \\(4QapocrLevi\textsuperscript{b})\end{tabular}&
   &
   &
   &
   \\
GrM-14364 &
   &
   &
   &
   &
   \\
GrM-14365 &
   &
   &
   &
   &
   \\ \hline
GrM-14571 &
  P330-Fr004 &
  \multirow{6}{*}{2159} &
  \multirow{6}{*}{22} &
  \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}346–316, \\ 204–165 BCE\end{tabular}} &
  \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}353–286, 229–217, \\ 211–104 BCE\end{tabular}} \\
GrM-14572 &
  \begin{tabular}[c]{@{}l@{}}4Q521 \\ (4QMessianic \\ Apocalypse)\end{tabular} &
   &
   &
   &
   \\
GrM-14377 &
   &
   &
   &
   &
   \\
GrM-14366 &
   &
   &
   &
   &
   \\ \hline
GrM-13393 &
  P107-Fr010 &
  \multirow{5}{*}{2151} &
  \multirow{5}{*}{21} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}344–320, \\ 202–157 BCE\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}351–294, 209–98, \\ 70–58 BCE\end{tabular}} \\
GrM-13394 &
\begin{tabular}[c]{@{}l@{}}4Q267 \\(4QDamascus\textsuperscript{b})\end{tabular} &
   &
   &
   &
   \\
GrM-14226 &
   &
   &
   &
   &
   \\
GrM-14227 &
   &
   &
   &
   &
   \\ \hline
GrM-14573 &
  P879-Fr001 &
  \multirow{4}{*}{1987} &
  \multirow{4}{*}{21} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}32–17 BCE, \\ 7–64 CE\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}41–9 BCE, \\ 1 BCE–81 CE, \\ 98–110 CE\end{tabular}} \\
GrM-14574 &
   \begin{tabular}[c]{@{}l@{}}Mur19 pap WrDiv\end{tabular}&
   &
   &
   &
   \\
GrM-14378 &
   &
   &
   &
   &
   \\
GrM-14379 &
   &
   &
   &
   &
   \\ \hline \hline

\end{longtable}}
\normalsize
\footnotetext{This fragment was previously unidentified, but see now for a positive identification~\cite{Tigchelaar2020B}.}

